Splatter-360: Generalizable 360$^{\circ}$ Gaussian Splatting for Wide-baseline Panoramic Images

Wide-baseline panoramic images are frequently used in applications like VR and simulations to minimize capturing labor costs and storage needs. However, synthesizing novel views from these panoramic images in real time remains a significant challenge, especially due to panoramic imagery's high resolution and inherent distortions. Although existing 3D Gaussian splatting (3DGS) methods can produce photo-realistic views under narrow baselines, they often overfit the training views when dealing with wide-baseline panoramic images due to the difficulty in learning precise geometry from sparse 360$^{\circ}$ views. This paper presents \textit{Splatter-360}, a novel end-to-end generalizable 3DGS framework designed to handle wide-baseline panoramic images. Unlike previous approaches, \textit{Splatter-360} performs multi-view matching directly in the spherical domain by constructing a spherical cost volume through a spherical sweep algorithm, enhancing the network's depth perception and geometry estimation. Additionally, we introduce a 3D-aware bi-projection encoder to mitigate the distortions inherent in panoramic images and integrate cross-view attention to improve feature interactions across multiple viewpoints. This enables robust 3D-aware feature representations and real-time rendering capabilities. Experimental results on the HM3D~\cite{hm3d} and Replica~\cite{replica} demonstrate that \textit{Splatter-360} significantly outperforms state-of-the-art NeRF and 3DGS methods (e.g., PanoGRF, MVSplat, DepthSplat, and HiSplat) in both synthesis quality and generalization performance for wide-baseline panoramic images. Code and trained models are available at \url{https://3d-aigc.github.io/Splatter-360/}.

==> image_tex/cmp.tex <==

\begin{figure*}[htbp]
\vspace{-10pt}
\centering
\scriptsize
\begin{tabular}{@{}c@{\,\,}c@{}c@{}c@{}c@{}c@{}c@{}c@{}}
\setlength{\tabcolsep}{10pt}
\\
\makecell[c]{
\includegraphics[trim={0px 0px 0px 0px}, clip, width=\resultsfigwidth]{results/cmp_replica_wide/gt_draw/6.jpg}
\\
\textit{Sample 1 (Replica)}
}
&
\cropcmpfifth{results/cmp_replica_wide/ibrnet/6.png} &
\cropcmpfifth{results/cmp_replica_wide/omnisyn/6.jpg} &
\cropcmpfifth{results/cmp_replica_wide/neuray/6.jpg} &
\cropcmpfifth{results/cmp_replica_wide/panogrf/6.jpg}
&
\cropcmpfifth{results/cmp_replica_wide/gt/6.jpg}  
\\
\makecell[c]{
\includegraphics[trim={0px 0px 0px 0px}, clip, width=\resultsfigwidth]{results/cmp_m3d/gt_draw/7.jpg}
\\
\textit{Sample 2 (Matterport3D)}
}
&

\cropcmpmt{results/cmp_m3d/ibrnet/7.png} &
\cropcmpmt{results/cmp_m3d/omnisyn/7.jpg} &
\cropcmpmt{results/cmp_m3d/neuray/7.jpg} &
\cropcmpmt{results/cmp_m3d/panogrf/7.jpg}
&
\cropcmpmt{results/cmp_m3d/gt/7.jpg}  
\\

 &IBRNet$^{*}$~\cite{ibrnet} & OmniSyn~\cite{omnisyn}&NeuRay$^{*}$~\cite{neuray} & \sysname{} & Ground Truth


% \\


% \makecell[c]{
% \includegraphics[trim={0px 0px 0px 0px}, clip, width=\resultsfigwidth]{results/cmp_residential/gt_draw/0.jpg}
% \\
% \textit{Sample 3 (Residential)}
% }
% & 
% \cropcmpsixth{results/cmp_residential/ibrnet/0.png} &
% \cropcmpsixth{results/cmp_residential/nerf/0.png} &
% \cropcmpsixth{results/cmp_residential/neuray/0.jpg} &
% \cropcmpsixth{results/cmp_residential/panogrf/0.jpg} &
% \cropcmpsixth{results/cmp_residential/gt/0.jpg} 

% \\

%  &IBRNet$^{*}$~\cite{ibrnet}& S-NeRF~\cite{nerf}&NeuRay$^{*}$~\cite{neuray} & \sysname{} & Ground Truth

\end{tabular}
\caption{Qualitative comparison on Replica and Matterport3D
 between IBRNet$^*$, OmniSyn, NeuRay$^*$ and \sysname{}.
}
\vspace{-5pt}
\label{fig:res-cmp}
\end{figure*}

==> image_tex/cmp1.tex <==
\newcommand{\resultsfigwidth}{1.5in}
\newcommand{\resultscropwidth}{0.75in}
% \renewcommand{\resultscropwidth}{0.79in}
% Define the crops here, individually for each image
\newcommand{\cropcmpfirst}[1]{
  \makecell{
  % left bottom right top
  % {"bbox": [218, 211, 584, 79]}
  \includegraphics[trim={68px 91px 679px 144px
}, clip, width=\resultscropwidth]{#1} \\
  % {"bbox": [4, 2, 845, 335]}
  \includegraphics[trim={391px 4px 455px 330px}, clip, width=\resultscropwidth]{#1} 
  }
}



% % {"bbox": [89, 95, 830, 312]}
% \newcommand{\cropcmpmatterport}[1]{
%   \makecell{
%   % left bottom right top
%   % {"bbox": [84, 75, 800, 297]}
%   \includegraphics[trim={84px 75px  800px 297px}, clip, width=\resultscropwidth]{#1}
  
%   \\
%   % {"bbox": [489, 80, 243, 140]}
%   \includegraphics[trim={489px 80px 243px 140px}, clip, width=\resultscropwidth]{#1} 
%   }
% }


% \newcommand{\resultsfigwidth}{1.5in}
% \newcommand{\resultscropwidth}{0.7in}
% \renewcommand{\resultscropwidth}{0.79in}
% Define the crops here, individually for each image

\begin{figure*}[htbp]
\vspace{-10pt}
\centering
\scriptsize
\begin{tabular}{@{}c@{\,\,}c@{}c@{}c@{}c@{}c@{}c@{}c@{}}
\setlength{\tabcolsep}{10pt}
% \begin{tabular}{@{}c@{\,\,}c@{\,\,}c@{}c@{}c@{}c@{}}
% \begin{tabular}{ccccc}
% \makecell[c]{
% \includegraphics[trim={0px 0px 0px 0px}, clip, width=\resultsfigwidth]{results/cmp_m3d/gt_draw/0.jpg}
% \\
% \textit{Sample 1}
% }
% & 
% \cropcmpfirst{results/cmp_m3d/gt/0.jpg} &
% \cropcmpfirst{results/cmp_m3d/ibrnet/0.png} &
% \cropcmpfirst{results/cmp_m3d/omnisyn/0.jpg} &
% \cropcmpfirst{results/cmp_m3d/neuray/0.jpg} &
% \cropcmpfirst{results/cmp_m3d/panogrf/0.jpg}

% \\
% \makecell[c]{
% \includegraphics[trim={0px 0px 0px 0px}, clip, width=\resultsfigwidth]{results/cmp_m3d/gt_draw/1.jpg}
% \\
% \textit{Sample 2}
% }
% & 
% \cropcmpsecond{results/cmp_m3d/gt/1.jpg} &
% \cropcmpsecond{results/cmp_m3d/ibrnet/1.png} &
% \cropcmpsecond{results/cmp_m3d/omnisyn/1.jpg} &
% \cropcmpsecond{results/cmp_m3d/neuray/1.jpg} &
% \cropcmpsecond{results/cmp_m3d/panogrf/1.jpg}
% \\
% \makecell[c]{
% \includegraphics[trim={0px 0px 0px 0px}, clip, width=\resultsfigwidth]{results/cmp_replica_wide/gt_draw/1.jpg}
% \\
% \textit{Sample 3}
% }
% & 
% \cropcmpthird{results/cmp_replica_wide/gt/1.jpg} &
% \cropcmpthird{results/cmp_replica_wide/ibrnet/1.png} &
% \cropcmpthird{results/cmp_replica_wide/omnisyn/1.jpg} &
% \cropcmpthird{results/cmp_replica_wide/neuray/1.jpg} &
% \cropcmpthird{results/cmp_replica_wide/panogrf/1.jpg}
% \\
% \makecell[c]{
% \includegraphics[trim={0px 0px 0px 0px}, clip, width=\resultsfigwidth]{cmp/gt/frl_apartment_5_0002/000001_erp_rect2.png}
% \\
% \textit{Sample 1}
% }
% &
% \cropcmpfirst{cmp/panogrf/frl_apartment_5_0002/000001_erp.png} &
% \cropcmpfirst{cmp/mvsplat/frl_apartment_5_0002/000001_erp.png} &
% \cropcmpfirst{cmp/ours/frl_apartment_5_0002/000001_erp.png} &
% \cropcmpfirst{cmp/gt/frl_apartment_5_0002/000001_erp_gt.png}  
\\
% \makecell[c]{
% \includegraphics[trim={0px 0px 0px 0px}, clip, width=\resultsfigwidth]{results/cmp_m3d/gt_draw/7.jpg}
% \\
% \textit{Sample 2 (Matterport3D)}
% }
% &

% \cropcmpmt{results/cmp_m3d/ibrnet/7.png} &
% \cropcmpmt{results/cmp_m3d/omnisyn/7.jpg} &
% \cropcmpmt{results/cmp_m3d/neuray/7.jpg} &
% \cropcmpmt{results/cmp_m3d/panogrf/7.jpg}
% &
% \cropcmpmt{results/cmp_m3d/gt/7.jpg}  
% \\

%  &IBRNet$^{*}$~\cite{ibrnet} & OmniSyn~\cite{omnisyn}&NeuRay$^{*}$~\cite{neuray} & \sysname{} & Ground Truth

\end{tabular}
\caption{Qualitative comparison on Replica and Matterport3D
 between IBRNet$^*$, OmniSyn, NeuRay$^*$ and \sysname{}.
}
\vspace{-5pt}
\label{fig:res-cmp}
\end{figure*}

==> image_tex/cmp2.tex <==
% 0.98in
% \newcommand{\macrowidth}{0.79in}
\newcommand{\resultsfigwidth}{1.5in}

%  (1024+10 + 256) = 1290 
% * 1.5 / 1024 
\newcommand{\resultscmpwidth}{1.8896in}
% 0.75 * 1.1 = 0.825
% 3.04 * 1.1 = 3.344
% 1054
% 1024
% \macrowidth
\begin{figure*}
%3.04
    \centering
    \begin{tabular}{@{}c@{\,}c@{\,}c@{\,}c@{\,}c@{}}
        \includegraphics[width=\resultsfigwidth] {cmp/gt/frl_apartment_5_0002/000001_erp_rect2.png} &
        
        \includegraphics[width=\resultscmpwidth]{cmp/panogrf/frl_apartment_5_0002/000001_erp_merge.png} & 
    	\includegraphics[width=\resultscmpwidth]{cmp/mvsplat/frl_apartment_5_0002/000001_erp_merge.png} &
    	\includegraphics[width=\resultscmpwidth]{cmp/ours/frl_apartment_5_0002/000001_erp_merge.png} &
    	\includegraphics[width=\resultscmpwidth]{cmp/gt/frl_apartment_5_0002/merge.png} \\
        

        % Second group
        \includegraphics[width=\resultsfigwidth] {cmp/gt/apartment_2_0001/000001_erp_rect2.png} &
        \includegraphics[width=\resultscmpwidth]{cmp/panogrf/apartment_2_0001/000001_erp_merge.png} & 
    	\includegraphics[width=\resultscmpwidth]{cmp/mvsplat/apartment_2_0001/000001_erp_merge.png} &
    	\includegraphics[width=\resultscmpwidth]{cmp/ours/apartment_2_0001/000001_erp_merge.png} &
    	\includegraphics[width=\resultscmpwidth]{cmp/gt/apartment_2_0001/merge.png} \\

        % 3rd group
        \includegraphics[width=\resultsfigwidth] {cmp/gt/hotel_0_0000/000000_erp_rect2.png} &
        \includegraphics[width=\resultscmpwidth]{cmp/panogrf/hotel_0_0000/000000_erp_merge.png} & 
    	\includegraphics[width=\resultscmpwidth]{cmp/mvsplat/hotel_0_0000/000000_erp_merge.png} &
    	\includegraphics[width=\resultscmpwidth]{cmp/ours/hotel_0_0000/000000_erp_merge.png} &
    	\includegraphics[width=\resultscmpwidth]{cmp/gt/hotel_0_0000/merge.png} \\

        % 4-th group
        \includegraphics[width=\resultsfigwidth] {cmp/gt/office_0_0000/000002_erp_rect2.png} &
        \includegraphics[width=\resultscmpwidth]{cmp/panogrf/office_0_0000/000002_erp_merge.png} & 
    	\includegraphics[width=\resultscmpwidth]{cmp/mvsplat/office_0_0000/000002_erp_merge.png} &
    	\includegraphics[width=\resultscmpwidth]{cmp/ours/office_0_0000/000002_erp_merge.png} &
    	\includegraphics[width=\resultscmpwidth]{cmp/gt/office_0_0000/merge.png} \\
        
        \small (a) Input views &
        \small (b) PanoGRF  &
        \small (c) MVSplat & 
        \small (d) Ours & 
        \small (e) Ground Truth \\
        
    \end{tabular}
    \caption{Novel view synthesis comparison between PanoGRF, MVSplat and \sysname{}.}
    \label{fig:replica_cmp}
    % \label{fig:cmp}
\end{figure*}

==> image_tex/cmp3.tex <==
% 0.98in
% \newcommand{\macrowidth}{0.79in}
\newcommand{\resultsfigwidth}{3.36in}
\newcommand{\resultscropwidth}{0.825in}
% 0.75 * 1.1 = 0.825
% 3.04 * 1.1 = 3.344
% 1054
% 1024
% \macrowidth
\begin{figure*}
%3.04
    \centering
    \begin{tabular}{@{}c@{\,}c@{\,}c@{\,}c@{\,}c@{}}
        \includegraphics[width=\resultsfigwidth] {cmp/gt/frl_apartment_5_0002/000001_erp_rect2.png} &
        
        \includegraphics[width=\resultscropwidth]{cmp/panogrf/frl_apartment_5_0002/000001_erp_merge.png} & 
    	\includegraphics[width=\resultscropwidth]{cmp/mvsplat/frl_apartment_5_0002/000001_erp_merge.png} &
    	\includegraphics[width=\resultscropwidth]{cmp/ours/frl_apartment_5_0002/000001_erp_merge.png} &
    	\includegraphics[width=\resultscropwidth]{cmp/gt/frl_apartment_5_0002/merge.png} \\
        

        % Second group
        \includegraphics[width=\resultsfigwidth] {cmp/gt/apartment_2_0001/000001_erp_rect2.png} &
        \includegraphics[width=\resultscropwidth]{cmp/panogrf/apartment_2_0001/000001_erp_merge.png} & 
    	\includegraphics[width=\resultscropwidth]{cmp/mvsplat/apartment_2_0001/000001_erp_merge.png} &
    	\includegraphics[width=\resultscropwidth]{cmp/ours/apartment_2_0001/000001_erp_merge.png} &
    	\includegraphics[width=\resultscropwidth]{cmp/gt/apartment_2_0001/merge.png} \\

        % 3rd group
        \includegraphics[width=\resultsfigwidth] {cmp/gt/hotel_0_0000/000000_erp_rect2.png} &
        \includegraphics[width=\resultscropwidth]{cmp/panogrf/hotel_0_0000/000000_erp_merge.png} & 
    	\includegraphics[width=\resultscropwidth]{cmp/mvsplat/hotel_0_0000/000000_erp_merge.png} &
    	\includegraphics[width=\resultscropwidth]{cmp/ours/hotel_0_0000/000000_erp_merge.png} &
    	\includegraphics[width=\resultscropwidth]{cmp/gt/hotel_0_0000/merge.png} \\

        % 4-th group
        \includegraphics[width=\resultsfigwidth] {cmp/gt/office_0_0000/000002_erp_rect2.png} &
        \includegraphics[width=\resultscropwidth]{cmp/panogrf/office_0_0000/000002_erp_merge.png} & 
    	\includegraphics[width=\resultscropwidth]{cmp/mvsplat/office_0_0000/000002_erp_merge.png} &
    	\includegraphics[width=\resultscropwidth]{cmp/ours/office_0_0000/000002_erp_merge.png} &
    	\includegraphics[width=\resultscropwidth]{cmp/gt/office_0_0000/merge.png} \\
        
        \small (a) Ground Truth Image, with Annotations &
        \small (b) PanoGRF  &
        \small (c) MVSplat & 
        \small (d) Ours & 
        \small (e) Ground Truth \\
        
    \end{tabular}
    \caption{Novel view synthesis comparison between PanoGRF, MVSplat and \sysname{}.}
    \label{fig:replica_cmp}
    % \label{fig:cmp}
\end{figure*}
